An efficient four-way coupled lattice Boltzmann - discrete element method for fully resolved simulations of particle-laden flows

A four-way coupling scheme for the direct numerical simulation of particle-laden flows is developed and analyzed. It employs a novel adaptive multi-relaxation time lattice Boltzmann method to simulate the fluid phase efficiently. The momentum exchange method is used to couple the fluid and the particulate phase. The particle interactions in normal and tangential direction are accounted for by a discrete element method using linear contact forces. All parameters of the scheme are studied and evaluated in detail and precise guidelines for their choice are developed. The development is based on several carefully selected calibration and validation tests of increasing physical complexity. It is found that a well-calibrated lubrication model is crucial to obtain the correct trajectories of a sphere colliding with a plane wall in a viscous fluid. For adequately resolving the collision dynamics it is found that the collision time must be stretched appropriately. The complete set of tests establishes a validation pipeline that can be universally applied to other fluid-particle coupling schemes providing a systematic methodology that can guide future developments.

==> numericalmethod.tex <==
\section{Numerical Method}
%\label{sec:numerical_method}

%\input{LBM}

%\input{RPD}

%\input{coupling}

%\input{completeAlgortihm}


==> obliqueDryWallCollision.tex <==
\section{Oblique collision of sphere with plane}

\subsection{Background}

\begin{itemize}
	\item test of tangential force model
	\item ours is very simple
\end{itemize}

\subsection{Description}

% currently only dry collision
In order to validate the tangential collision model, including the spring-damper model and the friction forces, we make use of a setup in which a sphere hits a plane in different angles.
By evaluating the resulting rebound angles, the simulations can be compared against the experimental findings from \cite{foerster1994} for the same setup.
A similar test has been carried out in \cite{biegert2017}, where it has been noted that the correct detection of sticking and slipping regimes is a key aspect for accurate results.
The impact ratio $\psi_{in} = u_{r,t}^{pre} / u_{r,n}$ is varied by changing velocity component that is tangential to the wall, i.e. $ u_{r,t}^{in}$, before the collision accordingly.
After the collision, the rebound ratio $\psi_{out} = u_{r,t}^{post} / u_{r,n}$ is evaluated, where the tangential velocity has contributions from translational and rotational velocities.
All velocities are measured at the particle's contact point with the wall.
We note that there is no surrounding fluid in this case and we do not consider gravitational forces.
Further parameters are $T_c = 60$, $\Delta t = 0.1$, $\mu_s = 0.8$, $\mu_d = 0.12$, $D_p=20$, $\rho_p=2.5$, $e=0.83$, $u_{r,n} = 0.02$.

%TODO add wet collision

\subsection{Results and discussion}

The results are shown in Fig.~\ref{fig:oblique_collision_test}, where a very good agreement with the experimental data can be seen.

%TODO add wet results


\begin{figure}[t]
	\centering	
	\input{figures/oblique_collision_test.pgf}
	\caption{Oblique collision of a sphere with a plane. Experimental data from \cite{foerster1994}. Data should be available from database.}
	\label{fig:oblique_collision_test}
\end{figure}

\begin{itemize}
	\item alternative would be the test case from \cite{costa2015}, with data (dry and wet) from \cite{joseph2004}
	\item other alternative would be sphere-sphere collision, with data from \cite{foerster1994}
\end{itemize}

